A Performance Study of Horizontally Explicit Vertically Implicit (HEVI) Time-Integrators for Non-Hydrostatic Atmospheric Models

We conduct a thorough study of different forms of horizontally explicit and vertically implicit (HEVI) time-integration strategies for the compressible Euler equations on spherical domains typical of nonhydrostatic global atmospheric applications. We compare the computational time and complexity of two nonlinear variants (NHEVI-GMRES and NHEVI-LU) and a linear variant (LHEVI). We report on the performance of these three variants for a number of additive Runge-Kutta Methods ranging in order of accuracy from second through fifth, and confirm the expected order of accuracy of the HEVI methods for each time-integrator. To gauge the maximum usable time-step of each HEVI method, we run simulations of a nonhydrostatic baroclinic instability for 100 days and then use this time-step to compare the time-to-solution of each method. The results show that NHEVI-LU is 2x faster than NHEVI-GMRES, and LHEVI is 5x faster than NHEVI-LU, for the idealized cases tested. The baroclinic instability and inertia-gravity wave simulations indicate that the optimal choice of time-integrator is LHEVI with either second or third order schemes, as both schemes yield similar time to solution and relative L2 error at their maximum usable time-steps. In the future, we will report on whether these results hold for more complex problems using, e.g., real atmospheric data and/or a higher model top typical of space weather applications.

==> sections/Balanced_Mountain.tex <==
% !TEX root = ../main_HEVI.tex

%----------------------------------------------------------------------------Moved into Spatial_Discretization Section
%\subsection{Static Balanced State with a Mountain}
%\label{sec:mountain}
%
%To compare the curl-invariant and cross-product metric terms, we use the mountain case from \cite{tomita:2004} with some of the parameters modified, i.e., the size of the mountain is bigger but we apply no initial wind velocity. The profile of the axisymmetric mountain is defined as follows
%\be
%  \mathrm{height} = \frac{h_m}{1+ \left( \frac{r}{a_m} \right)^2}
%\ee
% where $r = R_{e} \cos^{-1} \left( \cos \phi \cos \lambda \right)$ with $h_{m}=15$ km and $a_m=5000$ km, with the model top at $z_T = 30$ km. The profile of the mountain is shown in Fig.\ \ref{fig:results/Mountain/mountain_profile} and has been made artificially large (almost twice the height of Mount Everest) in order to stress the metric terms. The profile shown in the figure comes directly from the computational grid used for this test where $5 \times 5$ elements are used on each panel of the cubed-sphere grid \cite{ronchi:1996} along with 5 elements in the vertical using polynomial degree $N=4$ in all directions which results in an average grid resolution of 500 km in the horizontal and 1.25 km in the vertical where a terrain-following coordinate is used \cite{galchen:1975}.
% The grid is purposely coarse to test how well the metric terms perform in such resolution regimes.
%
%Figure  \ref{fig:results/Mountain/mass_loss} shows the mass loss for a 30-day simulation with data at a daily cadence; the mass loss is defined as
%\[
%\mathrm{Mass \, Loss} =\frac{ \abs{M(t) - M(0) }} { M(0) } 
%\]
%where
%\[
%M(t)= \int_{\Omega} \rho(t) d\Omega 
%\]
%for any time $t$ integrating along the global domain $\Omega$. The dashed red line in Fig.\ \ref{fig:results/Mountain/mass_loss} representing the cross-product metrics hovers on the order of $\order{10^{-5}}$ mass loss. In contrast, the solid blue line for the curl-invariant metrics conserves mass to machine double precision. 
%
%Although not shown, the baroclinic instability test conserves mass to machine double precision for the curl-invariant metrics for all 100-day simulations.
%\begin{figure}
%\begin{center}
%\begin{subfigure}{2.5in}
% \includegraphics[width=2.5in]{figures/Mountain/Mountain_Profile.png}
% \caption{Profile}
% \label{fig:results/Mountain/mountain_profile}
% \end{subfigure}
%\begin{subfigure}{2.5in}
%\includegraphics[width=2.5in]{figures/Mountain/Case142_Mass_Loss.png}
% \caption{Mass Loss}
% \label{fig:results/Mountain/mass_loss}
%\end{subfigure}
%\caption{Static Balanced Mountain. (a) Profile of mountain and (b) mass loss for a 30-day simulation comparing the curl-invariant and cross-product metrics.}
%\label{fig:results/Mountain}
%\end{center}
%\end{figure}
%

